Contextual Label Projection for Cross-Lingual Structured Prediction

Label projection, which involves obtaining translated labels and texts jointly, is essential for leveraging machine translation to facilitate cross-lingual transfer in structured prediction tasks. Prior research exploring label projection often compromise translation accuracy by favoring simplified label translation or relying solely on word-level alignments. In this paper, we introduce a novel label projection approach, CLaP, which translates text to the target language and performs contextual translation on the labels using the translated text as the context, ensuring better accuracy for the translated labels. We leverage instruction-tuned language models with multilingual capabilities as our contextual translator, imposing the constraint of the presence of translated labels in the translated text via instructions. We benchmark CLaP with other label projection techniques on zero-shot cross-lingual transfer across 39 languages on two representative structured prediction tasks - event argument extraction (EAE) and named entity recognition (NER), showing over 2.4 F1 improvement for EAE and 1.4 F1 improvement for NER. We further explore the applicability of CLaP on ten extremely low-resource languages to showcase its potential for cross-lingual structured prediction.

==> sections/expt.tex <==
\section{Experimental Setup}

In this section, we describe our experimental setup comprising the dataset, our evaluation setup, the baseline models, and the implementation details.

\subsection{Task and Dataset}

We choose two structure extraction downstream tasks of Event Argument Extraction (EAE) \cite{sundheim-1992-overview, hsu-etal-2023-tagprime} and Named Entity Recognition (NER) \tanmay{Need citations} for evaluating our label projection model.
EAE requires the extraction of text segments serving as arguments corresponding to an event and mapping them to their corresponding argument roles while NER aims to identify and categorize named entities from the input sentence.
We utilize the multilingual ACE dataset \cite{doddington-etal-2004-automatic} and the WikiANN \cite{pan-etal-2017-cross, rahimi-etal-2019-massively} for benchmarking EAE and NER respectively.
For both tasks, we consider the zero-shot cross-lingual transfer using English (\textit{en}) as the source language.
% In our work, we choose the representative structure extraction task as Event Argument Extraction (EAE) \cite{sundheim-1992-overview, hsu-etal-2023-tagprime, subburathinam-etal-2019-cross} which aims to extract text segments serving as arguments corresponding to an event and mapping them to their corresponding argument roles.
% The formal definition of the task is delineated in \S~\ref{sec:str-pred}.
% We utilize the multilingual EAE dataset of ACE \cite{doddington-etal-2004-automatic} as the benchmarking dataset and consider cross-lingual transfer in the zero-shot setting, where we do not use any supervised target language data (i.e. $\mathcal{D}_{tgt} = \phi$).
% Using ACE, we transfer cross-lingually from English (\textit{en}) to Arabic (\textit{ar}) and English (\textit{en}) to Chinese (\textit{zh}).
For ACE, we follow the pre-processing by \citet{wadden-etal-2019-entity} and \citet{huang-etal-2022-multilingual-generative} to retain 33 event types and 22 argument roles.
For WikiANN, we utilize pre-processing by XTREME \cite{XTREME}.
We provide the high-level statistics for these datasets in Table~\ref{tab:data-statistics} (detailed version in \S~\ref{sec:appendix-data-statistics}).
% Considering the zero-shot cross-lingual transfer scenario, the training and development sets are used from the source language (i.e. English), while the test datasets are used from the target languages (i.e. Arabic and Chinese).

% In our work, we choose the representative structure extraction task as Event Argument Extraction (EAE) \cite{sundheim-1992-overview, hsu-etal-2023-tagprime, subburathinam-etal-2019-cross} which aims to extract text segments serving as arguments corresponding to an event and mapping them to their corresponding argument roles.
% The formal definition of the task is delineated in \S~\ref{sec:str-pred}.
% We utilize the multilingual EAE dataset of ACE \cite{doddington-etal-2004-automatic} as the benchmarking dataset and consider cross-lingual transfer in the zero-shot setting, where we do not use any supervised target language data (i.e. $\mathcal{D}_{tgt} = \phi$).
% Using ACE, we transfer cross-lingually from English (\textit{en}) to Arabic (\textit{ar}) and English (\textit{en}) to Chinese (\textit{zh}).
% We follow the pre-processing by \citet{wadden-etal-2019-entity} and \citet{huang-etal-2022-multilingual-generative} to retain 33 event types and 22 argument roles and provide the final statistics for ACE in Table~\ref{tab:ace-statistics}.
% Considering the zero-shot cross-lingual transfer scenario, the training and development sets are used from the source language (i.e. English), while the test datasets are used from the target languages (i.e. Arabic and Chinese).

\begin{table}[t]
    \small
    \centering
    \begin{tabular}{lrr}
    \toprule
         & \textbf{ACE} & \textbf{WikiANN} \\
         \midrule
        \# Train Instances & $4,202$ & $20,000$ \\
        \# Dev Instances & $450$ & $10,000$ \\
        \# Avg. Test Instances & $194$ & $6,469$ \\
        \# Test Languages & $2$ & $39$ \\
    \bottomrule
    \end{tabular}
    \caption{High-level data statistics for ACE and WikiANN datasets for EAE and NER tasks respectively. \# = `number of' and Avg. = `average'.}
    \label{tab:data-statistics}
\end{table}

% \begin{table}[t]
%     \small
%     \centering
%     \setlength{\tabcolsep}{4.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lcc|cc}
%     \toprule
%          & \textbf{Train} & \textbf{Dev} & \multicolumn{2}{c}{\textbf{Test}} \\
%          Language & English & English & Arabic & Chinese \\
%     \midrule
%          \# Sentences & 17,172 & 923 & 272 & 482 \\
%          \# Events & 4,202 & 450 & 198 & 190 \\
%          \# Arguments & 4,859 & 605 & 287 & 336 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Data Statistics in terms of sentences, events, and arguments of the ACE dataset for the task of Event Argument Extraction (EAE). \# indicates `number of'.}
%     \label{tab:ace-statistics}
% \end{table}

\subsection{Evaluation Setup}

We conduct evaluation for the label projection task in two setups: (1) intrinsic evaluation and (2) extrinsic evaluation.
We describe these evaluations and their metrics below.

\subsubsection{Intrinsic Evaluation}

Intrinsic evaluation directly evaluates the label projection techniques in terms of accuracy and faithfulness of the translated labels.
\textbf{Accuracy} is measured in terms of translation quality by comparing the source labels with the translated labels ($\textbf{y} \leftrightarrow \textbf{y}^{tgt}$).
% \textbf{Accuracy} is measured in terms of translation quality by comparing a small sample\footnote{We choose 50 samples for this evaluation.} of labels in the source and target language ($\textbf{y} \leftrightarrow \textbf{y}^{tgt}$).
The translation quality is measured by native human speakers by relatively ranking the translated labels by the different techniques in terms of their translation quality.\footnote{We choose 50 samples for this evaluation.}
\textbf{Faithfulness} is the measure of the fulfillment of the label projection constraint.
It is measured simply as a percentage of datapoints when all the translated labels are present in the translated input sentence $\big( y^{tgt}_{m} \in x^{tgt} \quad \forall y^{tgt}_{m} \in \textbf{y}^{tgt} \big)$.

\subsubsection{Extrinsic Evaluation}

Extrinsic evaluation implicitly evaluates the label projection techniques for their ability to generate good-quality data for the translate-train application.
The quality of the generated data is measured as the F1 score of the model performance for the downstream tasks of EAE and NER.
For translate-train, we only retain the translated datapoints $(x^{tgt}, \textbf{y}^{tgt}, \textbf{r})$ that satisfy the label projection constraint (i.e. faithfulness) as part of the target pseudo-training data $\mathcal{D}^{tgt}_{src}$.
% Thus, a less faithful technique would yield a smaller-sized $\mathcal{D}^{tgt}_{src}$.
We train the downstream models on the concatenation of the source training data $\mathcal{D}_{src}$ and the label-projected target data $\mathcal{D}^{tgt}_{src}$.
% \footnote{Our ablation studies indicate that training on the concatenation of the datasets is better than training only on the target pseudo-training data.}

% \subsection{Structured Prediction Tasks and Datasets}

% We evaluate our approach on the structured prediction representative task of Event Argument Extraction (EAE)\ihung{add citation} which aims to extract text segments serving as arguments corresponding to an event and mapping them to their corresponding argument roles.
% The formal definition of the task is delineated in \S~\ref{sec:str-pred}.
% We utilize the multilingual EAE dataset of ACE \cite{doddington-etal-2004-automatic} as the benchmarking dataset and use F1 score as the main evaluation metric.
% We consider the more extreme case of zero-shot cross-lingual transfer, where we do not use any supervised target language data (i.e. $\mathcal{D}_{tgt} = \phi$.
% Using ACE, we transfer cross-lingually from English (\textit{en}) to Arabic (\textit{ar}) and English (\textit{en}) to Chinese (\textit{zh}).
% We follow the pre-processing by \citet{wadden-etal-2019-entity} to retain 33 event types and 22 argument roles.
% We provide the statistics for ACE in Table~\ref{tab:ace-statistics}.
% Considering the zero-shot cross-lingual transfer scenario, the training and development sets are used from the source language (i.e. \textit{en}), while the test datasets are used from the target languages (i.e. \textit{ar} and \textit{zh}).

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lcc|cc}
%     \toprule
%          & \textbf{Train} & \textbf{Dev} & \multicolumn{2}{c}{\textbf{Test}} \\
%          Language & en & en & ar & zh \\
%     \midrule
%          \# Sentences & 17,172 & 923 & 272 & 482 \\
%          \# Events & 4,202 & 450 & 198 & 190 \\
%          \# Arguments & 4,859 & 605 & 287 & 336 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Data Statistics in terms of sentences, events, and arguments of the ACE dataset for the task of Event Argument Extraction (EAE). \# indicates `number of'.}
%     \label{tab:ace-statistics}
% \end{table}

% \begin{table*}[ht]
%     \small
%     \centering
%     \setlength{\tabcolsep}{4.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lll|ccc|ccc}
%         \toprule
%         \multirow{2}{*}{\textbf{System 1}} & \multirow{2}{*}{\textbf{v/s}} & \multirow{2}{*}{\textbf{System 2}} & \multicolumn{3}{|c|}{\textbf{Arabic}} & \multicolumn{3}{c}{\textbf{Chinese}} \\ \cline{4-9}
%          & & & \textbf{System 1 win} & \textbf{Tie} & \textbf{System 2 win} & \textbf{System 1 win} & \textbf{Tie} & \textbf{System 2 win} \\
%         \midrule
%         \modelName & & Awesome-align & \textbf{32\%} & 60\% & 8\% & \textbf{52\%} & 46\% & 2\% \\
%         \modelName & & EasyProject & \textbf{78\%} & 12\% & 10\% & \textbf{58\%} & 36\% & 6\% \\
%         Awesome-align & & EasyProject & \textbf{60\%} & 22\% & 18\% & \textbf{35\%} & 36\% & 29\% \\
%         \bottomrule
%     \end{tabular}
%     \caption{A/B comparison of the various label projection techniques for accuracy evaluation for the many-to-many mBART translation model. Accuracy is measured in terms of the contextual translation quality of the labels by native human speakers. %Here, \textbf{S1} means System 1 is better, \textbf{S2} means System 2 is better, and \textbf{Tie} indicates both systems are similar quality. 
%     The better systems are highlighted in \textbf{bold}.}
%     \label{tab:accuracy-results}
% \end{table*}

% \begin{table*}[ht]
%     \small
%     \centering
%     \setlength{\tabcolsep}{4.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lll|ccc|ccc|ccc|ccc}
%         \toprule
%         \multirow{2}{*}{\textbf{System 1}} & \multirow{2}{*}{\textbf{v/s}} & \multirow{2}{*}{\textbf{System 2}} & \multicolumn{3}{|c|}{\textbf{Arabic}} & \multicolumn{3}{c|}{\textbf{Chinese}} & \multicolumn{3}{c|}{\textbf{Hindi}} & \multicolumn{3}{c}{\textbf{Spanish}} \\ \cline{4-15}
%          & & & \textbf{S1} & \textbf{Tie} & \textbf{S2} & \textbf{S1} & \textbf{Tie} & \textbf{S2} & \textbf{S1} & \textbf{Tie} & \textbf{S2} & \textbf{S1} & \textbf{Tie} & \textbf{S2} \\
%         \midrule
%         \modelName & & Awesome-align & \textbf{36\%} & 58\% & 6\% & \textbf{45\%} & 50\% & 5\% & \textbf{20\%} & 74\% & 6\% & \textbf{12\%} & 84\% & 4\% \\
%         \modelName & & EasyProject & \textbf{52\%} & 32\% & 16\% & \textbf{56\%} & 39\% & 5\% & \textbf{42\%} & 48\% & 10\% & \textbf{30\%} & 66\% & 4\% \\
%         \modelName & & Independent & 18\% & 60\% & \textbf{22\%} & 12\% & 71\% & \textbf{17\%} & \textbf{18\%} & 64\% & \textbf{18\%} & \textbf{24\%} & 68\% & 8\% \\
%         Independent & & Awesome-align & \textbf{44\%} & 42\% & 14\% & \textbf{39\%} & 57\% & 4\% & \textbf{28\%} & 60\% & 12\% & \textbf{20\%} & 64\% & 16\% \\
%         Independent & & EasyProject & \textbf{50\%} & 44\% & 6\% & \textbf{50\%} & 46\% & 4\% & \textbf{52\%} & 36\% & 12\% & \textbf{32\%} & 52\% & 16\% \\
%         Awesome-align & & EasyProject & \textbf{42\%} & 26\% & 32\% & \textbf{34\%} & 50\% & 16\% & \textbf{42\%} & 42\% & 16\% & \textbf{26\%} & 64\% & 10\% \\
%         \bottomrule
%     \end{tabular}
%     \caption{A/B comparison of the various label projection techniques for accuracy evaluation for the Google Translation model. Accuracy is measured as the label translation quality by native human speakers. Here, \textbf{S1} = System 1 is better, \textbf{S2} = System 2 is better, and \textbf{Tie} = similar quality. The better systems are highlighted in \textbf{bold}.}
%     \label{tab:accuracy-results}
% \end{table*}

\subsection{Baseline Models}
\label{sec:baseline_exp}

For baseline models, we compare against two previous label projection techniques:
\begin{itemize} [topsep=3pt, itemsep=-2pt, leftmargin=13pt]
    \item \textbf{Awesome-align} \cite{dou-neubig-2021-word}, a neural bilingual word alignment model, uses multilingual BERT \cite{devlin-etal-2019-bert} to find word similarities to derive word alignments, which are later used for label projection.
    \item \textbf{EasyProject} \cite{chen-etal-2023-frustratingly}, a recent marker-based translation technique, utilizes numbered square braces (e.g. [0] and [/0]) to mark the labels in the input sentence.
    The marked input sentence is translated and translated labels are retrieved using fuzzy-matching.
    % The transformed input sentence is then translated, and translated labels are retrieved using post-processing and fuzzy-matching.
\end{itemize}

\noindent Furthermore, we also compare with two simple yet strong ablative models:
\begin{itemize} [topsep=3pt, itemsep=-2pt, leftmargin=13pt]
    \item \textbf{Independent} translation uses the translation model $\mathcal{T}$ to independently (without any context of the input sentence) translate the source text labels to the target language (i.e. $\textbf{y}^{tgt} = \mathcal{T}(\textbf{y})$).
    % This method offers strong accuracy but poorer faithfulness as it doesn't impose any constraint on the translation.
    \item \textbf{Constrained} translation follows a \modelName's paradigm of contextual machine translation using a simple inference-time constraint.
    More specifically, it uses the translation model $\mathcal{T}$ to translate the labels $\textbf{y}$ while simultaneously limiting the generation vocabulary to the tokens in the translated sentence $x^{tgt}$.
    Since $\textbf{y}^{tgt}$ can only use tokens from $x^{tgt}$, it implicitly forces the model to be more faithful.
    We follow \citet{de-cao-etal-2022-multilingual, lu-etal-2022-summarization} for implementing these constraints.
    % \item \textbf{Constrained} translation, building atop the \textit{Independent} translation model, imposes an additional inference-time constraint to implicitly improve faithfulness of the translated labels. More specifically, $\mathcal{T}$ is limited to generate vocabulary of the text segment translations ($s^{tgt}$) to the space of tokens in the translated input sentence $x^{tgt}$.
    % This inference-time constraint implicitly forces the model to be more faithful in nature.
    % We follow \citet{de-cao-etal-2022-multilingual, lu-etal-2022-summarization} for implementing these constraints.
    % \tanmay{Should we mention this as our contribution/novelty as well? Like another way to do contextualized label projection}
\end{itemize}

% \begin{table}[t]
%     \small
%     \centering
%     \setlength{\tabcolsep}{4.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lcc}
%         \toprule
%          % & \multicolumn{2}{c}{\textbf{Faithfulness}} \\
%         \textbf{Techniques} & \textbf{Arabic} & \textbf{Chinese} \\
%         \midrule
%         Awesome-align & 69\% & \textbf{83\%} \\
%         EasyProject & 27\% & 29\% \\
%         \modelName & \textbf{74\%} & 81\% \\
%         \bottomrule
%     \end{tabular}
%     \caption{Faithfulness evaluation of the various label projection techniques as a percentage of the times the translated labels were present in the translated input sentence. Higher faithfulness is better and the best techniques are highlighted in \textbf{bold}.}
%     \label{tab:faithfulness-results}
% \end{table}

% \begin{table}[t]
%     \small
%     \centering
%     \setlength{\tabcolsep}{4.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lcc}
%         \toprule
%         \textbf{Techniques} & \textbf{EAE} & \textbf{NER} \\
%         \midrule
%         Independent & $35\%$ & $69\%$ \\
%         Awesome-align & $74\%$ & $93\%$ \\
%         EasyProject & $48\%$ & $92\%$ \\
%         \modelName &  & $79\%$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Faithfulness evaluation of the various label projection techniques for EAE and NER tasks as a percentage of the times the translated labels were present in the translated input sentence. Numbers are averaged over the languages for each task. Higher faithfulness is better and the best techniques are highlighted in \textbf{bold}.}
%     \label{tab:faithfulness-results}
% \end{table}

\begin{table*}[ht]
    \small
    \centering
    \setlength{\tabcolsep}{4.5pt}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l|l|cc|cc|cc|c}
        \toprule
         \multicolumn{2}{c|}{} & \multicolumn{2}{|c|}{\textbf{mBART}} & \multicolumn{2}{c|}{\textbf{mT5}} & \multicolumn{2}{c|}{\textbf{mT5+Copy}} & \textbf{Average} \\
         \multicolumn{2}{c|}{} & Arabic & Chinese & Arabic & Chinese & Arabic & Chinese \\ 
        \midrule
        \multicolumn{2}{l|}{Zero-shot} & 36.25 & 47.30 & 36.71 & 51.03 & 40.26 & 51.90 & 43.91 \\
        \multicolumn{2}{l|}{Supervised} & 60.69 & 66.38 & 61.41 & 68.62 & 63.15 & 69.67 & 64.99 \\ \midrule \midrule
        \multirow{5}{*}{\shortstack[l]{mBART-50 \\many-to-many}} & Awesome-align & \textbf{45.65} & 48.62 & 43.09 & 52.08 & 47.07 & 53.76 & 48.38 \\
        & EasyProject & 37.34 & \textbf{53.64} & 35.34 & 54.00 & 36.48 & 55.58 & 45.40 \\
        & Independent & 44.77 & 49.48 & 41.26 & 50.63 & 44.76 & 54.30 & 47.53 \\
        & Constrained & 44.48 & 51.24 & 42.30 & 53.54 & 45.58 & 55.59 & 48.79 \\ \cline{2-9}
        & \modelName & 45.49 & 52.04 & \textbf{44.83} & \textbf{54.66} & \textbf{48.17} & \textbf{56.92} & \textbf{50.35} \\
        \midrule
        \multirow{4}{*}{\shortstack[l]{Google Machine\\Translation}} & Awesome-align & 45.18 & 49.41 & \textbf{46.82} & 53.71 & 48.60 & 54.53 & 49.71 \\
        & EasyProject & 37.85 & 52.28 & 34.50 & 54.59 & 38.50 & 56.28 & 45.67 \\
        & Independent & 39.28 & 50.34 & 36.99 & 53.61 & 39.91 & 52.34 & 45.41 \\ \cline{2-9}
        & \modelName & \textbf{46.01} & \textbf{53.43} & 44.27 & \textbf{56.53} & \textbf{49.27} & \textbf{58.63} & \textbf{51.36} \\
        \bottomrule
    \end{tabular}
    \caption{Main Results in F1 score for zero-shot cross-lingual transfer on the ACE dataset using the mBART50 many-to-many and the Google machine translation as machine translators pairing with different label projection methods. We compare \modelName{} with Awesome-align~\cite{dou-neubig-2021-word}, EasyProject \cite{chen-etal-2023-frustratingly}, and two other ablative baselines introduced in Section~\ref{sec:baseline_exp}.
    We also present zero-shot and the supervised baselines as the lower and upper limits for reference. \textbf{Average} indicates the average across all models and target languages.}
    \label{tab:eae-results}
\end{table*}


\subsection{Model Implementations}

% \tanmay{Can make this more generic and discuss implementations of all models.}

% \modelName{} comprises a translation model $\mathcal{T}$ and a large language model $\mathcal{L}$.
For the translation model $\mathcal{T}$, we experiment with two models: (1) mBART-50 many-to-many (M2M) \cite{DBLP:conf/eacl/KongRCTGL21} and (2) Google Machine Translation (gmt).\footnote{\url{https://cloud.google.com/translate}}
For \modelName{}, we use the relatively smaller LLM Llama-2 \cite{touvron2023llama} with 13B parameters (i.e. \texttt{llama-2-13b}) as the $\mathcal{M}$ model.
For the prompt of $\mathcal{M}$, we use $n=2$ in-context examples.
For Awesome-align, we use the unsupervised version of their model as it gave better results.
For EasyProject, we do not train the translation model $\mathcal{T}$ for a fairer comparison with the other techniques.
For other settings of all the models, we use the default hyperparameters.

In terms of downstream models for intrinsic evaluation, we use the state-of-the-art model for zero-shot cross-lingual EAE: X-Gear \cite{huang-etal-2022-multilingual-generative}.
% The original X-Gear models explored two base multilingual models: mBART-50-large (mBART) \cite{DBLP:conf/eacl/KongRCTGL21} and the mT5-base (mT5) \cite{xue-etal-2021-mt5}.
% They also explored the usage of copy mechanism \cite{see2017get} to prompt the models to predict strings from the input sentence.
We explore three versions of the X-Gear model: mBART without copy (mBART), mT5 without copy (mT5), and mT5 with copy mechanism (mT5+Copy).
For NER, we use $\text{XLM-RoBERTa}_{\text{large}}$ \cite{conneau-etal-2020-unsupervised} and use the XTREME \cite{XTREME} setup for implementation.
\tanmay{to be updated}
Additional implementation details are mentioned in \S~\ref{sec:implementation-details}.
% We follow similar hyperparameter settings as the original work for training and testing the models.



==> sections/intro.tex <==
\section{Introduction}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.97\linewidth]{images/task-figure.pdf}
    \caption{Illustration of the task of \textit{label projection} from English to Chinese.
    Label projection converts sentences from a source to a target language while translating the associated labels jointly. Failures in this process occur when labels are either inaccurately translated or missing in the translated sentence in the target language.}
    \label{fig:label-projection-task}
    \vspace{-0.7em}
\end{figure}

Cross-lingual transfer in structure extraction tasks, such as named entity recognition, relation extraction, and event extraction, has gained considerable attention recently~\cite{huang-etal-2022-multilingual-generative, DBLP:conf/aaai/CaoJ00023, tedeschi-navigli-2022-multinerd, huguet-cabot-etal-2023-red,  DBLP:conf/aaai/FinckeAMB22, jenkins-etal-2023-massively, DBLP:conf/aaai/AhmadPC21}. It generalizes models trained in some source languages for use in other target languages, broadening the scope of these applications to more languages~\cite{XTREME, DBLP:conf/emnlp/ChenR21, subburathinam-etal-2019-cross, pouran-ben-veyseh-etal-2022-mee}.
% \textit{Label projection}, which jointly translates input sentences and obtains the translation of labels presented in the translated sentence, is a necessary step for cross-lingual transfer in structure extraction tasks if we want to leverage machine translators to generate pseudo-training data on target languages and help improve model's performance~\cite{xue-etal-2021-mt5, ruder-etal-2021-xtreme, yu-etal-2023-bridging}. As shown in Figure~\ref{fig:label-projection-task}, translated labels are the new learning target for models on target languages, which differs from simple classification tasks where the learning target is the same in the pseudo-training data and the source sentence~\cite{XTREME, chen-etal-2023-frustratingly}.
One effective and generic way to improve performance in cross-lingual transfer, called translate-train, is to leverage machine translators to generate pseudo-training data on target languages~\cite{xue-etal-2021-mt5, ruder-etal-2021-xtreme, yu-etal-2023-bridging}. 
However, applying this technique to structure extraction tasks necessitates a \textit{label projection} step, which involves jointly translating input sentences and labels~\cite{chen-etal-2023-frustratingly}.
As illustrated in Figure~\ref{fig:label-projection-task}, precise label projection requires not only accurate translation of the labels but also the presence of translated labels in the translated sentence.
This rigorous requirement on translating labels is different from  translate-train for basic classification tasks where mere sentence translation suffices~\cite{XTREME}. 


Prior works usually deal with label projection through two primary frameworks.
The first involves using word similarity to procure word alignments between the source and translated sentences~\cite{stengel-eskin-etal-2019-discriminative, akbik-etal-2015-generating, aminian-etal-2019-cross} and using them to map the source labels in the translated sentence.
% . The translated labels are then collected by processing and merging aligned word pairs from the labels in the source sentence.
The other framework performs machine translation on modified source sentences that incorporate label annotations in the source sentence using special markers~\cite{chen-etal-2023-frustratingly,  hennig-etal-2023-multitacred}.
Translated labels can be extracted if special markers are retained in the translated modified source sentences.
However, it is hard for the former approach to ensure \textit{accurate} label translation by merely using word alignments, as we will show in Section~\ref{sec:intrinsic-results}.
For the latter method, the quality of the translation is \textit{inherently compromised} due to the inclusion of markers~\cite{chen-etal-2023-frustratingly}. 
% Additionally, the efficacy of this method is highly contingent upon the robustness of the machine translation system.

% \kaiwei{Spend two paras. Introduce problem statement better and explain what you'll do to improve.}
% \violet{Try to improve the excitement more.}

In this work, we introduce \modelName{} (\textbf{C}ontextual \textbf{La}bel \textbf{P}rojection), which obtains projected label annotations in the target language by conducting contextual machine translation on the labels.
We first acquire the translation of the whole input sentence by any plug-and-play machine translation module.
Then, we leverage the idea of contextual machine translation~\cite{wong-etal-2020-contextual, voita-etal-2018-context} and use the translated input text as context to perform label translation, as shown in Figure~\ref{fig:methodology}(c).
Ensuring unmodified source sentences for translation better exploits machine translators and guarantees the quality of the translated sentence.
The usage of contextual machine translation strongly enhances the accuracy of the translated labels while preserving the presence of translated labels in the context.

We use an instruction-tuned language model with multilingual capabilities, Llama-2 model~\cite{touvron2023llama}, to execute contextual machine translation.
We encode the translated input sentence and the constraint for the presence of labels in the translated sentence as instructions in the model prompt. 
We select a representative structure extraction task - event argument extraction - as our testbed for the experiments, and project English training data to Chinese and Arabic using the ACE dataset \cite{doddington-etal-2004-automatic}.
Our intrinsic evaluation of the projected labels' quality shows that \modelName{} is preferable or comparable to baselines more than 90\% of the time in both languages.
Our extrinsic evaluation of applying translated data for zero-shot cross-lingual event argument extraction task using the translate-train technique demonstrates an average improvement of 2 to 2.5 F1 scores over other label projection baselines.
Finally, we provide qualitative examples showing how \modelName{} corrects the errors made by the other baseline techniques.




==> sections/results.tex <==
\section{Results}

We organize our results according to the two evaluation setups as below.

\subsection{Intrinsic Evaluation}
\label{sec:intrinsic-results}

We show the results comparing the label projection techniques of Awesome-align, EasyProject, and \modelName{} for accuracy and faithfulness in Table~\ref{tab:accuracy-results} and ~\ref{tab:faithfulness-results} respectively.
Accuracy evaluation is done by $5$ native bilingual speakers for Chinese, Arabic, Hindi, and Spanish.
We present the results as an A/B comparison of the different techniques in terms of their win rates (i.e. percentage when A is better than B).
\tanmay{Should we just report S1-S2?}
For faithfulness, we report the percentage of datapoints when all the labels of the sentence are present in the translated input sentence.
% \tanmay{To be completed}

In terms of accuracy (Table~\ref{tab:accuracy-results}), we observe a clear dominance of \modelName{} as it produces more accurate label translations than both the other techniques.
In fact, for 90\% cases, it is better or similar to the baseline technique.
% Awesome-align is better than EasyProject for Arabic while both are at par for Chinese.
In terms of faithfulness (Table~\ref{tab:faithfulness-results}), we note that \modelName{} and Awesome-align are similarly faithful while EasyProject relatively shows a poorer faithfulness score.
We note that the Awesome-align and EasyProject baselines can be less faithful owing to the absence of alignment for the labels or the absence of any markers in the translated sentence respectively.
Overall, intrinsic evaluation reveals that \modelName{} is a highly accurate and decently faithful model.
\tanmay{to be updated}

\subsection{Extrinsic Evaluation}

\paragraph{EAE} We present the results for the EAE task using M2M and GMT translation models in Table~\ref{tab:eae-results}.
For reference, we also include the zero-shot baseline\footnote{Reproduced numbers} (training on source data $\mathcal{D}_{src}$) and the supervised baseline (training on actual target data $\mathcal{D}_{tgt}$).
We exclude the Constrained baseline for GMT since it's a blackbox translation model.

% We present the main results for the extrinsic evaluation comparing \modelName{} with other baseline models for the Many-to-many-large-50 translation model (\textit{m2m}) and the Google Machine Translation model (\textit{gmt}) in Table~\ref{tab:all-results}.
% For reference, we also include the zero-shot baseline\footnote{Reproduced numbers} (X-Gear trained only on the source English training data $\mathcal{D}_{src}$) and the supervised baseline (X-Gear trained on the actual target language training data $\mathcal{D}_{tgt}$).
% We exclude the Constrained baseline for the \textit{gmt} translation model since it's a blackbox translation model and inference-time constraints can't be imposed on it.

% \begin{table*}[h]
%     \centering
%     \begin{tabular}{l|cc|cc|cc|c}
%         \toprule
%          & \multicolumn{2}{|c|}{\textbf{mBART}} & \multicolumn{2}{c|}{\textbf{mT5}} & \multicolumn{2}{c|}{\textbf{mT5+Copy}} & \textbf{Avg} \\
%          & ar & zh & ar & zh & ar & zh \\ 
%         \midrule
%         Zero-shot & 36.25 & 47.30 & 36.71 & 51.03 & 40.26 & 51.90 & 43.91 \\
%         Supervised & 60.69 & 66.38 & & & & \\ \hline
%         Awesome-align & 45.18 & 48.24 & \textbf{46.82} & 50.57 & 48.60 & 54.19 & 48.93 \\
%         EasyProject & 37.85 & 52.28 & 34.50 & 54.59 & 38.50 & 56.28 & 45.67 \\ \hline
%         Independent & 39.28 & 50.34 & 36.99 & 53.61 & 39.91 & 52.34 & 45.41 \\ \hline
%         \modelName & \textbf{46.01} & \textbf{53.43} & 44.27 & \textbf{56.53} & \textbf{49.27} & \textbf{58.63} & \textbf{51.36} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Main Results in F1 score for zero-shot cross-lingual transfer on the ACE dataset using the google translation model. \textbf{Avg} indicates the average across all models and target languages.}
%     \label{tab:gmt-ace-results}
% \end{table*}

% \ihung{Merge the two tables; remove line between independent and EasyProject}

Our results from Table~\ref{tab:eae-results} reveal how all the various translate-train techniques significantly improve over the simple zero-shot baseline.
Overall, \modelName{} performs the best amongst all translate-train techniques across various base models, languages, and translation models with an average improvement of $2$-$2.5$ F1 points over the next best baseline and an overall improvement of $6.5$-$7.5$ F1 points over the zero-shot baseline.

\begin{table*}[ht]
    \centering
    \small
    \setlength\tabcolsep{2pt}
    \begin{tabular}{l|cccccccccccccccccccc}
        \toprule
        Lang & af & ar & bg & bn & de & el & es & et & eu & fa & fi & fr & he & hi & hu & id & it & ja & jv & ka \\
        \midrule
        Zero-shot & $77.4$ & $48.1$ & $82.8$ & $77$ & $78.8$ & $80.6$ & $74.5$ & $78.7$ & $61.4$ & $69.2$ & $79.3$ & $79.4$ & $57.3$ & $70.6$ & $80.8$ & $53.1$ & $79.4$ & $19.1$ & $58.5$ & $72.3$ \\
        \hline
        Independent & \\
        Awesome-align & $77.9$ & $46$ & $81$ & $81.2$ & $78.8$ & $71.7$ & $65.3$ & $78$ & $66.8$ & $46.4$ & $77.4$ & $78.2$ & $55.3$ & $73.9$ & $77.4$ & $52.8$ & $79.3$ & $20.3$ & $56.3$ & $70.4$ \\
        EasyProject & $76.1$ & $34.4$ & $81$ & $78.6$ & $78.8$ & $69.3$ & $70.5$ & $73.9$ & $54.8$ & $49.1$ & $77.8$ & $78.8$ & $61.1$ & $73$ & $75.6$ & $51$ & $79$ & $41.3$ & $62.4$ & $66.4$ \\
        \modelName{} & \\
        \midrule
        & kk & ko & ml & mr & ms & my & nl & pt & ru & sw & ta & te & th & tl & tr & ur & vi & yo & zh & \textbf{Avg} \\
        \midrule
        Zero-shot & $51.9$ & $57.5$ & $66.4$ & $65.3$ & $53.4$ & $65.8$ & $83$ & $80$ & $74.2$ & $68.4$ & $60.3$ & $62.1$ & $0.4$ & $74.5$ & $65.6$ & $62.2$ & $75$ & $34.1$ & $24.6$ & $64.2$ \\
        \hline
        Independent & \\
        Awesome-align & $47.7$ & $57.7$ & $63.4$ & $62.4$ & $70.7$ & $54.1$ & $83$ & $75.8$ & $64.8$ & $70.1$ & $62.4$ & $55.4$ & $2.4$ & $80.9$ & $62.8$ & $53.7$ & $66.4$ & $61.5$ & $45.4$ & $63.5$ \\
        EasyProject & $31.7$ & $48.2$ & $56.5$ & $59.8$ & $71.7$ & $60.3$ & $81.9$ & $79.6$ & $66.3$ & $71.5$ & $53.2$ & $54.2$ & $11.4$ & $78.2$ & $66.8$ & $63.8$ & $65.6$ & $68.8$ & $42$ & $63.2$ \\
        \modelName{} & \\
        \bottomrule
    \end{tabular}
    \caption{Main NER Results}
    \label{tab:ner-results}
\end{table*}

\paragraph{NER} For NER, we present the main results for $XX$ languages using the GMT model in Table~\ref{tab:ner-results} along with the zero-shot baseline.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.92\textwidth]{images/Arab_Text_Testing.pdf}
%     \caption{Qualitative examples highlighting the error-cases of the baseline models along with the explanations for Arabic (ar) and Chinese (zh). We also show how \modelName{} performs better and fixes the errors. Here, \textbf{Tgt Lang} is the target language, "--" indicates the absence of the translated label.}
%     \label{fig:qual-study}
% \end{figure*}


\paragraph{Ablation Study}
Comparing the Independent model with \modelName{} in Table~\ref{tab:all-results}, we observe gains up to $3$-$6$ F1 points - highlighting the importance of meeting the faithfulness constraint.
Furthermore, \modelName{} outperforms the Constrained model by $2$ F1 points which underlines the importance of using a stronger instruction-tuned LM as $\mathcal{M}$ compared to using a simple inference-time constraint.
Overall, we also note how the paradigm of using contextual machine translation is better than previous works as the simple Constrained model outperforms Awesome-align and EasyProject baselines for the \textit{mmt} translation model.

% \begin{table*}[h]
%     \centering
%     \begin{tabular}{l|ccc|ccc|ccc}
%         \toprule
%          & \multicolumn{3}{|c|}{\textbf{XGear (mBART50)}} & \multicolumn{3}{c|}{\textbf{XGear (mT5)}} & \multicolumn{3}{c}{\textbf{XGear (mT5+Copy)}} \\
%          & ar & zh & es & ar & zh & es & ar & zh & es \\ 
%         \midrule
%         Zero-shot & 36.25 & 47.30 & 51.08 & 36.71 & 51.03 & 52.08 & 40.26 & 51.90 & 56.84 \\
%         Supervised & 60.69 & 66.38 & 63.32 & & & 65.66 & & & 66.13 \\ \hline
%         Awesome-align & \textbf{45.65} & 47.9 & \textbf{56.55} & 43.09 & 51.96 & \textbf{55.31} & 47.07* & 54.53 & \textbf{61.50} \\
%         Label Projection & 37.34 & \textbf{53.64} & 49.03 & 35.34 & 54 & 48.65 & 36.48 & 55.58 & 51.64 \\ \hline
%         Llama-2 Contextual & 45.49 & 52.04 & 53.84 & \textbf{44.83} & \textbf{54.66} & & \textbf{48.17} & \textbf{56.92} & 58.15 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Main Results Table for Many-to-many-large-50 Translation Model}
%     \label{tab:mmt-complete-results}
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \begin{tabular}{l|ccc|ccc|ccc}
%         \toprule
%          & \multicolumn{3}{|c|}{\textbf{XGear (mBART50)}} & \multicolumn{3}{c|}{\textbf{XGear (mT5)}} & \multicolumn{3}{c}{\textbf{XGear (mT5+Copy)}} \\
%          & ar & zh & es & ar & zh & es & ar & zh & es \\ 
%         \midrule
%         Zero-shot & 36.25 & 47.30 & 51.08 & 36.71 & 51.03 & 52.08 & 40.26 & 51.90 & 56.84 \\
%         Supervised & 60.69 & 66.38 & 63.32 & & & 65.66 & & & 66.13 \\ \hline
%         Awesome-align & 45.18 & 48.24 & 58.11 & \textbf{46.82} & 50.57 & 59.90 & 48.60 & 54.19 & 61.32 \\
%         Label Projection & 37.85 & 52.28 & 49.08 & 34.50 & 54.59 & 49.60 & 38.50 & 56.28 & 51.90 \\ \hline
%         Llama-2 Contextual & \textbf{46.01} & \textbf{53.43} & & 44.27 & \textbf{56.53} & & \textbf{49.27} & \textbf{58.63} & \\
%         \bottomrule
%     \end{tabular}
%     \caption{Main Results Table for Google Translate Translation Model}
%     \label{tab:gmt-complete-results}
% \end{table*}

% \subsection{Qualitative Analysis}

% % \begin{table*}[ht]
% %     \centering
% %     \begin{tabular}{p{7.3cm}ll|l|p{1.8cm}}
% %         \toprule
% %         \textbf{Source} & \textbf{Source} & \textbf{Target} & \multirow{2}{*}{\textbf{Technique}} & \textbf{Translated} \\
% %         % \multicolumn{2}{c|}{\textbf{Source}} & \multirow{2}{*}{\textbf{Technique}} & \\
% %         \textbf{Sentence} & \textbf{Label} & \textbf{Lang} & & \textbf{Label} \\
% %         \midrule
% %         % \multirow{2}{*}{\textbf{System 1}}
% %         \multirow{3}{7.3cm}{abbas was convicted in absentia by an italian court and sentenced to five life terms in prison.} & \multirow{3}{*}{court} & \multirow{3}{*}{ar} & Awesome-align & \ara{أبيس} \\ 
% %         & & & EasyProject & - \\ 
% %         & & & \modelName & \ara{المحكمة} \\
% %         \midrule
% %         \multirow{3}{7.3cm}{But unilaterally, or worse leading a coalition featuring tyrannies, effect such change remains a bad idea, Iraq's elections notwithstanding.} & \multirow{3}{*}{Iraq} & \multirow{3}{*}{zh} & Awesome-align & \zh{伊拉} \\ 
% %         & & & EasyProject & \zh{尽管伊拉克} \\ 
% %         & & & \modelName & \zh{伊拉克} \\
% %         \bottomrule
% %     \end{tabular}
% %     \caption{Qualitative examples highlighting the error-cases of the baseline models and how \modelName{} performs better. Here, \textbf{Target Lang} is the target language.}
% %     \label{tab:qual-study}
% % \end{table*}

% Diving deeper, we qualitatively study typical error cases for the translated labels by different label projection techniques.
% In the fifty examples of studies for each language, we found that EasyProject has around 50\% percentage of the time predicting nothing due to markers dropped in the translated sentence. This is also attributed to the low faithfulness scores in Table~\ref{tab:faithfulness-results}.
% For Awesome-align, the majority of errors they make are duplications of words or incomplete label translations, similar to the observation presented in \cite{chen-etal-2023-frustratingly}.
% This is because it is hard for the word-alignment module to decide alignments between sub-words, leading to over-alignment or under-alignment.
% We show two examples comprising the source sentence and the label translated into Arabic and Chinese in Figure~\ref{fig:qual-study}.
% The typical errors for EasyProject can be found in the Arabic example, while the Chinese example also demonstrates the typical incomplete predictions made by Awesome-align.
% Additionally, in the case of Chinese, extra characters (i.e. \zh{尽管}) are predicted by EasyProject since the markers are incorrectly placed in the translated sentence.
% In both cases, we show how \modelName{} makes accurate predictions and is more robust in maintaining accurate label translations.

% \subsection{Translate-Test Analysis}

% Mainly discuss EAE experiments + NER on a couple of languages for translate-test

% \subsection{Case Study: Challenging Examples}

% Choose longer length datapoints and report on 2-4 languages

% \subsection{Low-data Analysis}

% Can show results on 10\% NER data

% Fig 2 - single column
% Tab 2 + 3 -> plot
% Sec 4 + 5 -> intersparse + Sec 5 - Analysis
% Remove constrained as baseline + MMT as translation model -> Push as an ablation/analysis -> Tab 4 becomes smaller/single column

% Sec 2.2 -> Introduce translate-test. Mainly focus on translate-train (since less error propagation) + divert about to Sec 5
